Differential topology of the spaces of asymptotically stable vector fields and Lyapunov functions

We study the topology of the space of all smooth asymptotically stable vector fields on $\mathbb{R}^n$, as well as the space of all proper smooth Lyapunov functions for such vector fields. We prove that both spaces are path-connected and simply connected when $n\neq 4,5$ and weakly contractible when $n\leq 3$. Moreover, both spaces have the weak homotopy type of the nonlinear Grassmannian of submanifolds of $\mathbb{R}^n$ diffeomorphic to the $n$-disc. The proofs rely on Lyapunov theory and differential topology, such as the work of Smale and Perelman on the generalized Poincar\'{e} conjecture and results of Smale, Cerf, and Hatcher on the topology of diffeomorphism groups of discs. Applications include a partial answer to a question of Conley, a parametric Hartman-Grobman theorem for nonyperbolic but asymptotically stable equilibria, and a parametric Morse lemma for degenerate minima. We also study the related topics of hyperbolic equilibria, Morse minima, and relative homotopy groups of the space of asymptotically stable vector fields inside the space of those vanishing at a single point.

==> Inputs/app-pseudoisotopy-spheres-feb-4-before-trying-to-streamline-evaluate-derivative-argument.tex <==
The goal of this appendix is to explain the proof Theorem~\ref{th:pseudoisotopy} from results readily available in the literature.
The results employed are standard techniques used in the study of diffeomorphism groups, for which we freely refer to the lecture notes of S. Kupers \cite{kupers2019lectures}, and landmark results concerning the topology of (i) the diffeomorphism groups of the $2$-sphere by Smale \cite{smale1959diffeomorphisms} and the $3$-sphere by Hatcher \cite{hatcher1983proof}, and (ii) the pseudoisotopy spaces of high-dimensional simply connected manifolds by Cerf \cite{cerf1970stratification}.

Recall: a \concept{pseudoisotopy} of a compact $C^\infty$ manifold $M$ is a $C^\infty$ diffeomorphism of $M\times I$ that is the identity on $M\times \{0\}$. 
Let $\P(M)\subset \Diff(M\times I)$ denote the \concept{pseudoisotopy space} of all pseudoisotopies equipped with the $C^\infty$ topology.
If $f_1\in \Diff(M)$ and there is $f\in \P(M)$ with $f_1=f|_{M\times\{1\}}$, then $f_1$ is \concept{pseudoisotopic to the identity}.
Cerf proved the \concept{pseudoisotopy theorem} \cite[Thm~0]{cerf1970stratification}:
\begin{Th}[Cerf]\label{th:cerf}
Let $M$ be a compact smooth manifold. 
Assume that $M$ is simply connected and $\dim(M)\geq 5$. 
Then $\P(M)$ is path-connected.
\end{Th}

\begin{Rem}\label{rem:pseudoisotopy-implies-isotopy}
Theorem~\ref{th:cerf} is equivalent to the assertion that, for any $M$ as in its statement, ``pseudoisotopy implies isotopy''. In fact, since any isotopy $h_t$ from $\id_M$ to $f_1\in \Diff(M)$ gives rise to the ``level-preserving'' pseudoisotopy $(x,t)\mapsto (h_t(x),t)$, $f_1$ is pseudoisotopic to the identity if and only if $f_1$ is isotopic to the identity.
\end{Rem}

Theorem~\ref{th:cerf} implies the case $k=1$ and $n\geq 6$ of Theorem~\ref{th:pseudoisotopy}.
To establish the case $n\leq 3$, we use the following combination of results of Smale and Hatcher:
\begin{Th}[Smale, Hatcher]\label{app:th:diff-disk-rel-bd}
For $n=1,2,3$, $\Diff_\partial (D^n)$ is weakly contractible.
\end{Th}
In detail, Theorem~\ref{app:th:diff-disk-rel-bd} follows from an elementary convexity argument for $n=1$ \cite[Thm~3.2.1]{kupers2019lectures}, was proved for $n=2$ by Smale (\cite[Thm~B]{smale1959diffeomorphisms}, \cite[sec.~7.1]{kupers2019lectures}), and for  $n=3$ follows from Hatcher's proof of the Smale conjecture that $\Diff(S^3)$ deformation retracts onto the orthogonal group $O(4)$ \cite[p.~604]{hatcher1983proof}.

We use Theorem~\ref{app:th:diff-disk-rel-bd} in the proofs of both Theorem~\ref{th:pseudoisotopy} and the next lemma.

\begin{Lem}\label{app:lem:deriv-eval-htpy-equiv}
For $n=1,2,3$,  the ``evaluate derivative at $0$'' map $\Diff(D^n)\to \GL(n)$ defined by $f\mapsto D_0 f$ is a weak homotopy equivalence.
\end{Lem}

\begin{proof}
Let $\GS\colon \GL(n)\to  O(n)$ be the smooth homotopy equivalence obtained from applying the Gram-Schmidt orthonormalization procedure beginning from the first column.
Define a continuous map $p\colon \Diff(\sph^{n-1})\to O(n)$ by
\begin{equation}\label{eq:p-map}
p(f)= \GS(f(e_1),D_{e_1}f(e_2),\ldots, D_{e_1}f(e_{n})),
\end{equation}
where $e_1, \ldots, e_n$ is the standard orthonormal basis of $\R^n$.

Define $G \coloneqq p^{-1}(I_{n}) \subset \Diff(\sph^{n-1})$ to  be those diffeomorphisms that fix $e_1$ and whose derivatives at $e_1$ also fix the standard orthonormal tangent frame $e_2,\ldots, e_n$.
Note  that  $\sigma\colon O(n)\to 
\Diff(\sph^{n-1})$ defined by $\sigma(R)(x)=Rx$ is a continuous section of $p$.
Observe that $O(n) \times G\to \Diff(\sph^{n-1})$ defined by $(R,f)\mapsto \sigma(R)\circ f$  and $\Diff(\sph^{n-1})\to O(n) \times G$ defined by
\begin{equation}\label{eq:homeo-product}
f \mapsto (p(f),\sigma(p(f))^{-1}\circ f )
\end{equation}
are homeomorphisms and mutual inverses (cf. \cite[sec.~7.3]{kupers2019lectures}).

Parametrized isotopy extension implies that the restriction  
\begin{equation}\label{eq:restriction}
r \colon \Diff(D^n)\to \Diff(\sph^{n-1})	
\end{equation}
 is a fibration with fiber $\Diff_{\partial}(D^n)$ over the identity \cite[p.~70]{kupers2019lectures}, so Theorem~\ref{app:th:diff-disk-rel-bd} and the long exact sequence of homotopy groups imply that \eqref{eq:restriction} is a weak homotopy equivalence.

Identifying $\Diff_\partial(D^{n-1})$ with those diffeomorphisms of $\sph^{n-1}$ equal to the identity on the hemisphere opposite $e_1$, the inclusion $\Diff_\partial(D^{n-1})\hookrightarrow G$ is  a weak homotopy equivalence by scaling outwards \cite[sec.~4.1]{kupers2019lectures}.
Since \eqref{eq:homeo-product} is a homeomorphism and $\Diff_\partial(\Diff(D^{n-1}))$ is weakly contractible by Theorem~\ref{app:th:diff-disk-rel-bd} again, it follows that $p\colon \Diff(\sph^{n-1})\to O(n)$ and hence also $p\circ r\colon \Diff(D^n)\to O(n)$ are weak homotopy equivalences.
Since $p\circ r$ is straight-line homotopic to the time-$0$ map of the homotopy $H\colon I \times \Diff(D^n)\to O(n)$ defined by
$$H_t(f)= \GS(D_{t\cdot e_1}f(e_1),D_{t\cdot e_1}f(e_2),\ldots, D_{t\cdot e_1}f(e_{n})),$$
it follows that $H_0\colon \Diff(D^n)\to O(n)$ is a weak homotopy equivalence.
Finally, since
\begin{align*}
H_0(f)&=\GS(D_0f(e_1),\ldots, D_nf(e_n))
\end{align*}
and $\GS\colon \GL(n)\to O(n)$ is a homotopy equivalence, we  see that the evaluation map $\Diff(D^n)\to \GL(n)$ given by $f\mapsto D_0 f$ is a weak homotopy equivalence.
\end{proof}

The following proof of Theorem~\ref{th:pseudoisotopy}, restated here, uses Lemma~\ref{app:lem:deriv-eval-htpy-equiv} and was suggested by \'Alvaro del Pino G\'omez.

\MK{commented out theorem below}
%\ThmSmaleCerfHatcher*

\begin{proof}
Theorem~\ref{th:cerf} yields case (ii) since $\sph^{n-1}$ is simply connected for $n>2$.

It remains to establish case (i), so consider $n=1,2,3$ and the diagram
\begin{equation*}
	\begin{tikzcd}
		\P(S^{n-1})\approx \Diff_{B^n}(D^n)\arrow[r,hook] & \Diff(D^{n}) \arrow[d,"\rho",swap] \arrow[r, "\simeq"] & \GL(n) \arrow[d, "="]\\
		& \Emb(B^{n},D^{n}) \arrow[r, swap, "\simeq"] & \GL(n)
	\end{tikzcd}.
\end{equation*}
Here $B^n =\frac{1}{2}D^n\subset D^n$ is the closed ball of radius $\frac{1}{2}$, $\Diff_{B^n}(D^n)\subset \Diff(D^n)$ are those diffeomorphisms restricting to the identity on $B^n$, $\Emb(B^n, D^n)$ is the space of $C^\infty$ embeddings $B^n\hookrightarrow \interior{D^n}$ equipped with the $C^\infty$ topology, $\rho$ is the restriction map $\rho(f)=f|_{B^n}$, the left horizontal arrow is the inclusion of the fiber of $\rho$ over the inclusion $B^n\hookrightarrow D^n$, the right vertical arrow is the identity, and the two right horizontal arrows are both the ``evaluate derivative at $0$'' maps $f\mapsto D_0 f$.

The two right horizontal arrows are weak homotopy equivalences by scaling outward for the bottom map and Lemma~\ref{app:lem:deriv-eval-htpy-equiv} for the top map.
Since the square is commutative, this implies that $\rho$ is a weak homotopy equivalence.
Since $\rho$ is also a fibration by parametrized isotopy extension \cite[p.~70]{kupers2019lectures}, the long exact sequence of homotopy groups implies that $\P(S^{n-1})$ is weakly contractible, or $\pi_{k-1}(\P(\sph^{n-1}))=\{*\}$ for all $k\in \N_{\geq 1}$.
\end{proof}


==> Inputs/app-pseudoisotopy-spheres.tex <==
The goal of this appendix is to explain the proof Theorem~\ref{th:pseudoisotopy} from results readily available in the literature.
The results employed are standard techniques used in the study of diffeomorphism groups, for which we freely refer to the lecture notes of S. Kupers \cite{kupers2019lectures}, and landmark results concerning the topology of (i) the diffeomorphism groups of the $2$-sphere by Smale \cite{smale1959diffeomorphisms} and the $3$-sphere by Hatcher \cite{hatcher1983proof}, and (ii) the pseudoisotopy spaces of high-dimensional simply connected manifolds by Cerf \cite{cerf1970stratification}.

Recall: a \concept{pseudoisotopy} of a compact $C^\infty$ manifold $M$ is a $C^\infty$ diffeomorphism of $M\times I$ that is the identity on $M\times \{0\}$. 
Let $\P(M)\subset \Diff(M\times I)$ denote the \concept{pseudoisotopy space} of all pseudoisotopies equipped with the $C^\infty$ topology.
If $f_1\in \Diff(M)$ and there is $f\in \P(M)$ with $f_1=f|_{M\times\{1\}}$, then $f_1$ is \concept{pseudoisotopic to the identity}.
Cerf proved the \concept{pseudoisotopy theorem} \cite[Thm~0]{cerf1970stratification}:
\begin{Th}[Cerf]\label{th:cerf}
Let $M$ be a compact smooth manifold. 
Assume that $M$ is simply connected and $\dim(M)\geq 5$. 
Then $\P(M)$ is path-connected.
\end{Th}

\begin{Rem}\label{rem:pseudoisotopy-implies-isotopy}
Theorem~\ref{th:cerf} is equivalent to the assertion that, for any $M$ as in its statement, ``pseudoisotopy implies isotopy''. In fact, since any isotopy $h_t$ from $\id_M$ to $f_1\in \Diff(M)$ gives rise to the ``level-preserving'' pseudoisotopy $(x,t)\mapsto (h_t(x),t)$, $f_1$ is pseudoisotopic to the identity if and only if $f_1$ is isotopic to the identity.
\end{Rem}

Theorem~\ref{th:cerf} implies the case $k=1$ and $n\geq 6$ of Theorem~\ref{th:pseudoisotopy}.
To establish the case $n\leq 3$, we use the following combination of results of Smale and Hatcher:
\begin{Th}[Smale, Hatcher]\label{app:th:diff-disk-rel-bd}
For $n=1,2,3$, $\Diff_\partial (D^n)$ is weakly contractible.
\end{Th}
In detail, Theorem~\ref{app:th:diff-disk-rel-bd} follows from an elementary convexity argument for $n=1$ \cite[Thm~3.2.1]{kupers2019lectures}, was proved for $n=2$ by Smale (\cite[Thm~B]{smale1959diffeomorphisms}, \cite[sec.~7.1]{kupers2019lectures}), and for  $n=3$ follows from Hatcher's proof of the Smale conjecture that $\Diff(S^3)$ deformation retracts onto the orthogonal group $O(4)$ \cite[p.~604]{hatcher1983proof}.

We use Theorem~\ref{app:th:diff-disk-rel-bd} in the proofs of both Theorem~\ref{th:pseudoisotopy} and the next lemma.

\begin{Lem}\label{app:lem:deriv-eval-htpy-equiv}
For $n=1,2,3$,  the ``evaluate derivative at $0$'' map $\Diff(D^n)\to \GL(n)$ defined by $f\mapsto D_0 f$ is a weak homotopy equivalence.
\end{Lem}

\begin{proof}
Let $\GS\colon \GL(n)\to  O(n)$ be the smooth homotopy equivalence obtained from applying the Gram-Schmidt orthonormalization procedure beginning from the first column.
Define a continuous map $p\colon \Diff(\sph^{n-1})\to O(n)$ by
\begin{equation}\label{eq:p-map}
p(f)= \GS(f(e_1),D_{e_1}f(e_2),\ldots, D_{e_1}f(e_{n})),
\end{equation}
where $e_1, \ldots, e_n$ is the standard orthonormal basis of $\R^n$.

Define $G \coloneqq p^{-1}(I_{n}) \subset \Diff(\sph^{n-1})$ to  be those diffeomorphisms that fix $e_1$ and whose derivatives at $e_1$ also fix the standard orthonormal tangent frame $e_2,\ldots, e_n$.
Note  that  $\sigma\colon O(n)\to 
\Diff(\sph^{n-1})$ defined by $\sigma(R)(x)=Rx$ is a continuous section of $p$.
Observe that $O(n) \times G\to \Diff(\sph^{n-1})$ defined by $(R,f)\mapsto \sigma(R)\circ f$  and $\Diff(\sph^{n-1})\to O(n) \times G$ defined by
\begin{equation}\label{eq:homeo-product}
f \mapsto (p(f),\sigma(p(f))^{-1}\circ f )
\end{equation}
are homeomorphisms and mutual inverses (cf. \cite[sec.~7.3]{kupers2019lectures}).

Parametrized isotopy extension implies that the restriction  
\begin{equation}\label{eq:restriction}
r \colon \Diff(D^n)\to \Diff(\sph^{n-1})	
\end{equation}
 is a fibration with fiber $\Diff_{\partial}(D^n)$ over the identity \cite[p.~70]{kupers2019lectures}, so Theorem~\ref{app:th:diff-disk-rel-bd} and the long exact sequence of homotopy groups imply that \eqref{eq:restriction} is a weak homotopy equivalence.

Identifying $\Diff_\partial(D^{n-1})$ with those diffeomorphisms of $\sph^{n-1}$ equal to the identity on the hemisphere opposite $e_1$, the inclusion $\Diff_\partial(D^{n-1})\hookrightarrow G$ is  a weak homotopy equivalence by scaling outwards \cite[sec.~4.1]{kupers2019lectures}.
Since \eqref{eq:homeo-product} is a homeomorphism and $\Diff_\partial(\Diff(D^{n-1}))$ is weakly contractible by Theorem~\ref{app:th:diff-disk-rel-bd} again, it follows that $p\colon \Diff(\sph^{n-1})\to O(n)$ and hence also $p\circ r\colon \Diff(D^n)\to O(n)$ are weak homotopy equivalences.
Since $p\circ r$ is straight-line homotopic to the time-$0$ map of the homotopy $H\colon I \times \Diff(D^n)\to O(n)$ defined by
$$H_t(f)= \GS(D_{t\cdot e_1}f(e_1),D_{t\cdot e_1}f(e_2),\ldots, D_{t\cdot e_1}f(e_{n})),$$
it follows that $H_0\colon \Diff(D^n)\to O(n)$ is a weak homotopy equivalence.
Finally, since
\begin{align*}
H_0(f)&=\GS(D_0f(e_1),\ldots, D_nf(e_n))
\end{align*}
and $\GS\colon \GL(n)\to O(n)$ is a homotopy equivalence, we  see that the evaluation map $\Diff(D^n)\to \GL(n)$ given by $f\mapsto D_0 f$ is a weak homotopy equivalence.
\end{proof}

The following proof of Theorem~\ref{th:pseudoisotopy}, restated here, uses Lemma~\ref{app:lem:deriv-eval-htpy-equiv} and was suggested by \'Alvaro del Pino G\'omez.

\MK{commented out theorem below}
%\ThmSmaleCerfHatcher*

\begin{proof}
Theorem~\ref{th:cerf} yields case (ii) since $\sph^{n-1}$ is simply connected for $n>2$.

It remains to establish case (i), so consider $n=1,2,3$ and the diagram
\begin{equation*}
	\begin{tikzcd}
		\P(S^{n-1})\approx \Diff_{B^n}(D^n)\arrow[r,hook] & \Diff(D^{n}) \arrow[d,"\rho",swap] \arrow[r, "\simeq"] & \GL(n) \arrow[d, "="]\\
		& \Emb(B^{n},D^{n}) \arrow[r, swap, "\simeq"] & \GL(n)
	\end{tikzcd}.
\end{equation*}
Here $B^n =\frac{1}{2}D^n\subset D^n$ is the closed ball of radius $\frac{1}{2}$, $\Diff_{B^n}(D^n)\subset \Diff(D^n)$ are those diffeomorphisms restricting to the identity on $B^n$, $\Emb(B^n, D^n)$ is the space of $C^\infty$ embeddings $B^n\hookrightarrow \interior{D^n}$ equipped with the $C^\infty$ topology, $\rho$ is the restriction map $\rho(f)=f|_{B^n}$, the left horizontal arrow is the inclusion of the fiber of $\rho$ over the inclusion $B^n\hookrightarrow D^n$, the right vertical arrow is the identity, and the two right horizontal arrows are both the ``evaluate derivative at $0$'' maps $f\mapsto D_0 f$.

The two right horizontal arrows are weak homotopy equivalences by scaling outward for the bottom map and Lemma~\ref{app:lem:deriv-eval-htpy-equiv} for the top map.
Since the square is commutative, this implies that $\rho$ is a weak homotopy equivalence.
Since $\rho$ is also a fibration by parametrized isotopy extension \cite[p.~70]{kupers2019lectures}, the long exact sequence of homotopy groups implies that $\P(S^{n-1})$ is weakly contractible, or $\pi_{k-1}(\P(\sph^{n-1}))=\{*\}$ for all $k\in \N_{\geq 1}$.
\end{proof}


==> Inputs/commutative-diagram-with-nonlinear-grassmannian.tex <==
\begin{equation*}
	\begin{tikzcd}
		\U_0(D^n,\R^n)\\
		\fun_0^\infty(\R^n) \arrow["p"]{u} \arrow[hookrightarrow]{r} \arrow[hookrightarrow]{d} & \fun^\infty(\R^n) \arrow["-\nabla"]{r}\arrow[hookrightarrow]{d} & \stab^\infty(\R^n) \arrow[hookleftarrow]{r}\arrow[hookrightarrow]{d} &  \stab_0^\infty(\R^n) \arrow[hookleftarrow]{r}\arrow[hookrightarrow]{d}  & \stabc_0^\infty(\R^n) \arrow[hookrightarrow]{r} \arrow[hookrightarrow]{d}& \stabc^\infty(\R^n) \arrow[hookrightarrow]{d}\\
		\fun_0^{r+1}(\R^n) \arrow[hookrightarrow]{r} \arrow[hookrightarrow]{d} & \fun^{r+1}(\R^n) \arrow["-\nabla"]{r}\arrow[hookrightarrow]{d} \arrow[hookrightarrow]{d} & \stab^r(\R^n) \arrow[hookleftarrow]{r} & \stab_0^r(\R^n) \arrow[hookleftarrow]{r} & \stabc_0^r(\R^n) \arrow[hookrightarrow]{r} & \stabc^r(\R^n)\\
		\fun_0^r(\R^n) \arrow[hookrightarrow]{r} & \fun^r(\R^n)
	\end{tikzcd}
\end{equation*}

==> Inputs/commutative-diagram-without-nonlinear-grassmannian.tex <==
\begin{equation}\label{cd:comm-diag-without-nonlinear-grassmannian}
	\begin{tikzcd}
		\fun_0^1(\R^n) \arrow[hookrightarrow]{r} \arrow[hookrightarrow]{d}  & \fun_0^2(\R^n)\arrow[hookrightarrow]{r} \arrow[hookrightarrow]{d}  & \arrow[hookrightarrow]{r} \cdots \arrow[hookrightarrow]{r}\arrow[hookrightarrow]{d} 	&	\fun_0^{r+1}(\R^n)\arrow[hookrightarrow]{r}\arrow[hookrightarrow]{d}	& 	\fun_0^\infty(\R^n)  \arrow[hookrightarrow]{d} \\
		\fun^1(\R^n) \arrow[hookrightarrow]{r} \arrow[bend right]{u} & \fun^2(\R^n)\arrow[hookrightarrow]{r} \arrow["-\nabla"]{d} \arrow[bend right]{u}& \arrow[hookrightarrow]{r} \cdots \arrow[hookrightarrow]{r} \arrow["-\nabla"]{d} \arrow[bend right]{u}	&	\fun^{r+1}(\R^n)\arrow[hookrightarrow]{r}\arrow["-\nabla"]{d} \arrow[bend right]{u}	& 	\fun^\infty(\R^n) \arrow["-\nabla"]{d} \arrow[bend right]{u} \\
		& \stab^1(\R^n) \arrow[hookrightarrow]{r} \arrow[bend right]{d} & \cdots	\arrow[hookrightarrow]{r} \arrow[bend right]{d} & \stab^r(\R^n)  \arrow[hookrightarrow]{r} \arrow[bend right]{d} & \stab^\infty(\R^n) \arrow[bend right]{d} \\
		& \stab_0^1(\R^n) \arrow[hookrightarrow]{r} \arrow[hookrightarrow]{u}  & \cdots	\arrow[hookrightarrow]{r} \arrow[hookrightarrow]{u}& \stab_0^r(\R^n)  \arrow[hookrightarrow]{r} \arrow[hookrightarrow]{u} & \stab_0^\infty(\R^n) \arrow[hookrightarrow]{u}
	\end{tikzcd}
\end{equation}
